HSVI can solve zero-sum Partially Observable Stochastic Games

State-of-the-art methods for solving 2-player zero-sum imperfect information games rely on linear programming or regret minimization, though not on dynamic programming (DP) or heuristic search (HS), while the latter are often at the core of state-of-the-art solvers for other sequential decision-making problems. In partially observable or collaborative settings (e.g., POMDPs and Dec- POMDPs), DP and HS require introducing an appropriate statistic that induces a fully observable problem as well as bounding (convex) approximators of the optimal value function. This approach has succeeded in some subclasses of 2-player zero-sum partially observable stochastic games (zs- POSGs) as well, but how to apply it in the general case still remains an open question. We answer it by (i) rigorously defining an equivalent game to work with, (ii) proving mathematical properties of the optimal value function that allow deriving bounds that come with solution strategies, (iii) proposing for the first time an HSVI-like solver that provably converges to an $\epsilon$-optimal solution in finite time, and (iv) empirically analyzing it. This opens the door to a novel family of promising approaches complementing those relying on linear programming or iterative methods.

==> Makefile <==
TARGETS = extended.pdf theoretic-graph.pdf
DEPS_DIR = .deps
LATEXMK = latexmk -recorder -use-make -deps \
	-e 'warn qq(In Makefile, turn off custom dependencies);' \
	-e '@cus_dep_list = ();' \
	-e 'show_cus_dep();'

all : $(TARGETS)
$(foreach file,$(TARGETS),$(eval -include $(DEPS_DIR)/$(file)P))

$(DEPS_DIR) :
	mkdir $@

%.pdf : %.tex Makefile
	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
	-$(LATEXMK) -pdf -deps-out=$(DEPS_DIR)/$@P $<
	./check-tex.sh $(DEPS_DIR)/$@P
	./clean-deps.sh $(DEPS_DIR)/$@P
	./check-length.sh $<

theoretic-graph.pdf: theoretic-graph.sh article.tex body.tex appendix.tex
	./theoretic-graph.sh article.tex
	@echo evince theoretic-graph.pdf

rebuttal:
	./check-rebuttal.sh

biblio:
	latexmk -pdf article.tex
	latexmk -pdf extended.tex
	#latexmk -pdf diapos.tex
	#cat article.aux |sed -e 's/abx@aux@cite/citation/g' > article2.aux
	./make-biblio.sh extended.aux

ARX = ArXiv
arXiv:
	@rm -rf $(ARX)
	@mkdir $(ARX)
	@cp -r figures/ $(ARX)/
	@cp -r tikz/ $(ARX)/
	@cp arxiv-a4.sty $(ARX)/
	@cp table.tex $(ARX)/
	@latexpand --expand-bbl extended.bbl extended.tex -o $(ARX)/extended.tex
	@cp makefile-camera-ready $(ARX)/Makefile
	@cp clean-deps.sh $(ARX)/
	@cp slashbox.sty $(ARX)/
	@#$(foreach fig, $(shell grep "includegraphics" *.tex  | cut -d \{ -f 2 | cut -d \} -f 1), /bin/cp -rfvL ./figures/$(fig) $(ARX)/figures/;)
	@# note the final semi-colon in the last command


clean :
	rm -f *~ *bbl *.dot
	latexmk -c

veryclean:
	rm -f *~ .deps/* *.bbl figures/*.bak *.dot
	rm -rf $(ARX)
	latexmk -C


==> checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\addcontentsline{toc}{section}{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? %
    \answerYes{} %
  \item Did you describe the limitations of your work? %
    \answerYes{\em One limitation is that we did not tried all likely
      improvements of our work (see \Cref{sec|discussion}). %
      Also, our approach is currently outperformed by Sequence Form LP
      (\Cref{sec|XPs}), while modern applications rely on CFR-based
      approaches (\Cref{sec|introduction}).} %
  \item Did you discuss any potential negative societal impacts of your work? %
    \answerYes{\em We point out in \Cref{sec|XPs} that, ``while solving zsPOSGs
      may have both positive and negative impacts
      \citep{BroBakLerQon-nips20}, this implementation only tackles
      small problems.''}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} %
  \item Did you include complete proofs of all theoretical results?
    \answerYes{} %
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? %
    \answerYes{}%\em %
      % \olivier{On compte bien le faire :) {\bf Ajouter Licence (MIT?) via gitlab.}} \\ %
    %   \olivier{Ça devient trop compliqué toutes ces branches sur le dépôt git, non ? %
    %     Ne faudrait-il pas faire du ménage (après la deadline) pour que d'autres qu'Aurélien puissent s'y retrouver ?}
    %   %
    % }
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? %
    \answerYes{}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)? %
    \answerNA{\em Our algorithm is not randomized. %
      Note: Two of the algorithms used as references are randomized, but the available results rely on a single run.}
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
\item If your work uses existing assets, did you cite the creators?
  \answerYes{\em As explained in \Cref{sec|XPs}, we use Wiggers'
    implementation of the Sequence Form LP solver.}
  \item Did you mention the license of the assets?
    \answerNo{\em This implementation is currently unreleased and unlicensed.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{\em Our own source code is provided as supplemental material under MIT license.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{\em We do not use any dataset.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> extended.tex <==
\def\extended{true}

\input{article.tex}

% [Olivier] One line to tell emacs to use French spelling:
% Local IspellDict: American


==> tikz/matching_pennies.tex <==
\tikzset{
% Two node styles for game trees: solid and hollow
solid node/.style={circle,draw,inner sep=1.5,fill=black},
hollow node/.style={circle,draw,inner sep=1.5}
}

\begin{tikzpicture}[scale=1.5,font=\footnotesize]
% Specify spacing for each level of the tree
\tikzstyle{level 1}=[level distance=15mm,sibling distance=35mm]
\tikzstyle{level 2}=[level distance=15mm,sibling distance=7.5mm]
\tikzstyle{level 3}=[level distance=15mm,sibling distance=4.5mm]
% The Tree
\node(0)[solid node,label=above:{$P1$}]{}
child{node(1)[circle]{$s_h$}
child{node(3)[hollow node,label=left:{$2$},label=right:{\tiny{sh}}]{} 
%
%
child{node[hollow node,label=below:{2}]{} edge from parent node[left]{\tiny{*,h}}}
child{node[hollow node,label=below:{-1}]{} edge from parent node[left]{\tiny{*,t}}}
%
%
edge from parent node[left]{\tiny{$h,h$}}
}
child{node(4)[hollow node,label=right:{$-1$},label=left:{\tiny{sh}}]{}
%
child{node[hollow node,label=below:{2}]{} edge from parent node[left]{\tiny{*,h}}}
child{node[hollow node,label=below:{-1}]{} edge from parent node[left]{\tiny{*,t}}}
%
edge from parent node[left]{\tiny{$h,t$}}}
%
%
%
%
child{node(7)[hollow node,label=left:{$2$},label=right:{\tiny{st}}]{} 
%
%
child{node[hollow node,label=below:{-1}]{} edge from parent node[left]{\tiny{*,h}}}
child{node[hollow node,label=below:{1}]{} edge from parent node[left]{\tiny{*,t}}}
%
%
edge from parent node[left]{\tiny{$t,h$}}
}
child{node(8)[hollow node,label=right:{$-1$},label=left:{\tiny{st}}]{}
%
child{node[hollow node,label=below:{-1}]{} edge from parent node[left]{\tiny{*,h}}}
child{node[hollow node,label=below:{1}]{} edge from parent node[left]{\tiny{*,t}}}
%
edge from parent node[right]{\tiny{$t,t$}}}
edge from parent node[left,xshift=-3]{$Head,*$}
}
%
%
%
%
child{node(2)[circle]{$s_t$}
child{node(5)[hollow node,label=left:{$-1$},label=right:{\tiny{sh}}]{} 
%
%
child{node[hollow node,label=below:{2}]{} edge from parent node[left]{\tiny{*,h}}}
child{node[hollow node,label=below:{-1}]{} edge from parent node[left]{\tiny{*,t}}}
%
%
edge from parent node[left]{\tiny{$h,h$}}
}
child{node(6)[hollow node,label=right:{$1$},label=left:{\tiny{sh}}]{}
%
child{node[hollow node,label=below:{2}]{} edge from parent node[left]{\tiny{*,h}}}
child{node[hollow node,label=below:{-1}]{} edge from parent node[left]{\tiny{*,t}}}
%
edge from parent node[left]{\tiny{$h,t$}}
}
%
%
%
%
child{node(9)[hollow node,label=left:{$-1$},label=right:{\tiny{st}}]{} 
%
%
child{node[hollow node,label=below:{-1}]{} edge from parent node[left]{\tiny{*,h}}}
child{node[hollow node,label=below:{1}]{} edge from parent node[left]{\tiny{*,t}}}
%
%
edge from parent node[left]{\tiny{$t,h$}}
}
child{node(10)[hollow node,label=right:{$1$},label=left:{\tiny{st}}]{}
%
child{node[hollow node,label=below:{-1}]{} edge from parent node[left]{\tiny{*,h}}}
child{node[hollow node,label=below:{1}]{} edge from parent node[left]{\tiny{*,t}}}
%
edge from parent node[right]{\tiny{$t,t$}}
}
edge from parent node[left,xshift=-3]{$Tail,*$}
};
% information set
\draw[dashed,rounded corners=10]($(1) + (-.2,.25)$)rectangle($(2) +(.2,-.25)$);
% specify mover at 2nd information set
\node at ($(1)!.5!(2)$) {nodes indistinguishable to $P2$};
%
%
\draw[dashed,rounded corners=5,fill=blue!20, fill opacity = .25]($(3) + (-.15,.125)$)rectangle($(4) +(.15,-.125)$);
\draw[dashed,rounded corners=5,fill=blue!20, fill opacity = .25]($(5) + (-.15,.125)$)rectangle($(6) +(.15,-.125)$);
\draw[dashed,rounded corners=5,fill=orange!20, fill opacity = .25]($(7) + (-.15,.125)$)rectangle($(8) +(.15,-.125)$);
\draw[dashed,rounded corners=5,fill=orange!20, fill opacity = .25]($(9) + (-.15,.125)$)rectangle($(10) +(.15,-.125)$);

% specify mover at 2nd information set
\end{tikzpicture}

